FlowCam: Training Generalizable 3D Radiance Fields without Camera Poses via Pixel-Aligned Scene Flow

Reconstruction of 3D neural fields from posed images has emerged as a promising method for self-supervised representation learning. The key challenge preventing the deployment of these 3D scene learners on large-scale video data is their dependence on precise camera poses from structure-from-motion, which is prohibitively expensive to run at scale. We propose a method that jointly reconstructs camera poses and 3D neural scene representations online and in a single forward pass. We estimate poses by first lifting frame-to-frame optical flow to 3D scene flow via differentiable rendering, preserving locality and shift-equivariance of the image processing backbone. SE(3) camera pose estimation is then performed via a weighted least-squares fit to the scene flow field. This formulation enables us to jointly supervise pose estimation and a generalizable neural scene representation via re-rendering the input video, and thus, train end-to-end and fully self-supervised on real-world video datasets. We demonstrate that our method performs robustly on diverse, real-world video, notably on sequences traditionally challenging to optimization-based pose estimation techniques.

==> figText/co3d_result.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/co3d}
    
    \caption{\textbf{Results on generalization on CO3D.} Our approach is able to render novels views with higher quality than all baselines on both hydrants-only setting (top row) and the more challenging 10-category setting (bottom row). }
    \label{fig:co3d}
\end{figure*}

==> figText/hydrant_nvs.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
  %\vspace{-5pt}
  \centering
  \includegraphics[width=0.45\textwidth]{figs/novel_view_hydrant.pdf}
  \caption{\textbf{Feed-forward Novel View Synthesis}: Even without any scene-specific finetuning, our estimated poses and rendered novel views are reasonable. See Fig \ref{fig:overfitting} for an example where we additionally finetune before rendering for even sharper details.}
  \label{fig:hydrant_nvs}
  %\vspace{-10pt}
\end{wrapfigure}

==> figText/kitti.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/kitti.pdf}
    \caption{
    \textbf{Generalizable novel view synthesis results on KITTI, RealEstate10K, and CO3D.} Our approach is able to render novels views with higher quality than all baselines, without poses. PixelNeRF is provided as a posed reference to mark the upper bound on view synthesis. 
    }
    
    \label{fig:realestate}
\end{figure*}

==> figText/learned_geometry.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/learned_geometry.pdf}
    \caption{\textbf{Learned geometry.} Our model's expected ray termination depth illustrates the unsupervised geometry learned by our model. We show samples for the challenging CO3D dataset. 
    %
    }
    \label{fig:depth}
\end{figure}


==> figText/orbslam_comp.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{figs/orbslam_comp.pdf}
  \caption{\textbf{Our Method is More Robust than ORB-SLAM3}: Our method is more robust than per-scene optimization methods, thanks to our learned prior. We plot a sequence where ORB-SLAM3 succeeds and another where it fails to register any poses.}
  \label{fig:orbslam_comp}
\end{wrapfigure}

==> figText/skip_robustness.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/frame_skip_robustness.pdf}
    \caption{\textbf{Skip Robustnes.} Our model degrades performs well even with large camera transformations and degrades gracefully.
    %
    }
    \label{fig:depth}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
% \usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{wrapfig}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

\newcommand{\ours}[1]{\textcolor{cyan}{OURS}\xspace}
\newcommand{\VS}[1]{{\bf\textcolor{blue}{Vincent: #1}}}
\newcommand{\AT}[1]{{\bf\textcolor{orange}{Ayush: #1}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}




\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\ssect}[1]{\S~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}
\newcommand{\alg}[1]{Algorithm~\ref{#1}}


\definecolor{tabbestcolor}{rgb}{0.785, 0.851, 0.969}
\def \best {\cellcolor{tabbestcolor!85}}
\def \sbest {\cellcolor{tabbestcolor!30}}

\DeclareMathOperator*{\argmin}{arg\,min}
